Learning Symmetric and Low-energy Locomotion

Learning locomotion skills is a challenging problem. To generate realistic and smooth locomotion, existing methods use motion capture, finite state machines or morphology-specific knowledge to guide the motion generation algorithms. Deep reinforcement learning (DRL) is a promising approach for the automatic creation of locomotion control. Indeed, a standard benchmark for DRL is to automatically create a running controller for a biped character from a simple reward function. Although several different DRL algorithms can successfully create a running controller, the resulting motions usually look nothing like a real runner. This paper takes a minimalist learning approach to the locomotion problem, without the use of motion examples, finite state machines, or morphology-specific knowledge. We introduce two modifications to the DRL approach that, when used together, produce locomotion behaviors that are symmetric, low-energy, and much closer to that of a real person. First, we introduce a new term to the loss function (not the reward function) that encourages symmetric actions. Second, we introduce a new curriculum learning method that provides modulated physical assistance to help the character with left/right balance and forward movement. The algorithm automatically computes appropriate assistance to the character and gradually relaxes this assistance, so that eventually the character learns to move entirely without help. Because our method does not make use of motion capture data, it can be applied to a variety of character morphologies. We demonstrate locomotion controllers for the lower half of a biped, a full humanoid, a quadruped, and a hexapod. Our results show that learned policies are able to produce symmetric, low-energy gaits. In addition, speed-appropriate gait patterns emerge without any guidance from motion examples or contact planning.

==> method.tex <==
\section{Assistance Controller}
\label{sec:assist_contr}

A successful locomotion controller involves delicate balance among various aspects, including propelling forward, balancing, keeping upright posture, conserving energy, etc. Directly learning a policy to achieve these is difficult and only limited results can be obtained with careful tuning of the reward function. 

The idea behind our Assistance Controller (AC) is to decouple the learning goals by providing external forces to assist the agent in achieving a subset of them. Specifically, AC provides two types of assistance forces, the lateral balancing force and the propelling force, which corresponds to the two vital aspects in locomotion. The lateral balancing force is applied along the frontal axis of the character, which tries to keep the character from tipping off to the side, while the propelling force is applied along sagittal axis, which pushes the character forward to reach the desired velocity. With the assistance forces, the agent can focus on learning to balance in the sagittal plane as well as keeping the energy consumption low. We find that this is a much easier problem to solve than the full locomotion task. 

The Assistance Controller can potentially take different forms as long as it can successfully fulfill the designated assistance role. For example, one can train a control policy to serve as the Assistance Controller using Reinforcement Learning, or formulate hard constraints in the dynamic equations. In this work, we represent the AC use the stable proportional-derivative (SPD) controller \cite{tan2011stable}, where we set the reference position in frontal direction to be $0$ for the lateral balancing force and the reference velocity in sagittal direction to be the desired velocity $v^*$ for the propelling force. SPD controller provides us a few advantages over the other alternatives. First, it does not require any pre-training and can be applied to any character morphology with little tuning. In addition, it provides a smooth assistance in the state space, which facilitates learning. Finally, it is unconditionally stable, allowing us to use large controller gains without introducing instability. The strength of the Assistance Controller can be modulated through the proportional and derivative gains. These are then the quantities we adjust during the curriculum update step, and the goal of learning is to achieve successful locomotion with the controller gains reducing to $0$. The assistance forces are applied at the character's pelvis or thorax. We find our system insensitive to the exact location of application, as long as it is close to the main section of the body.

\section{Mirror Symmetry Loss}
\label{sec:mirror_sym_loss}

Imaging a person standing next to a floor stand mirror and trying to grab a hat using the right hand. If we look into the mirror, we will find that his/her left hand is doing the same task, with all the actions mirrored. More generally speaking, for a character with symmetric morphology, the action it takes in certain pose should be the mirrored version of the action taken when it is in the mirrored pose. Mathematically, this property can be expressed as: 

\begin{equation}
\pi_{\theta}(\vc{s}_t) = \Psi_a(\pi_{\theta}(\Psi_o(\vc{s}_t))),
\end{equation}
where $\Psi_a(\cdot)$ and $\Psi_o(\cdot)$ maps actions and states to their mirrored version respectively. This property should hold for policies of any character with symmetric layouts. Ideally, the Reinforcement Learning algorithm should search only in the space of controllers with such property for these problems. However, enforcing this analytically is non-trivial as typical controllers treat different parts of the character independently. As a result, the trained controller tends to use asymmetric control strategies and generates unnatural motion. To encourage the algorithm in searching policies with mirror symmetry property, we formulate it as a soft constraint:

\begin{equation}
L_{mirror}(\theta) = \sum_{i=0}^B||\pi_{\theta}(\vc{s}_i) - \Psi_a(\pi_{\theta}(\Psi_o(\vc{s}_i)))||_2,
\end{equation}
where $B$ is the number of simulation samples per iteration. We use $20,000$ samples in all of our examples. Since the Mirror Symmetry Loss is differentiable w.r.t the policy parameters $\theta$, it can be combined with the standard reinforcement learning objective and optimized using any gradient-based RL algorithm.

\section{Policy Learning}
\label{sec:policy_learning}

We model the locomotion task as a Markov Decision Process (MDP). A MDP can be defined as a tuple $(S, A, R, \rho_0, T, \gamma)$, where $S$ is the state space, $A$ is the action space, $R$ is the reward function, $\rho_0$ is the initial state distribution, $T:S \times A \mapsto S$ is the transition function and $\gamma$ is the discount factor.

The \textit{Value Function} of a policy starting from some state $\vc{s}_0$ is defined as:

\begin{equation}
V(\vc{s}_0) = \mathbb{E}_{\vc{a}_0{,}\vc{s}_1{,}...}[\sum_{i=0}^N \gamma^i R(\vc{s}_i, \vc{a}_i)],
\end{equation}
where $\vc{a}_{i+1} {\sim} \pi(\vc{s}_i)$ and $\vc{s}_{i+1}{\sim}T(\vc{s}_i, \vc{a}_i)$. Value function measures the return of a trajectory starting from $\vc{s}_0$ and follows the policy $\pi_\theta$. We also define \textit{Q Function}:

\begin{equation}
Q(\vc{s}_0, \vc{a}) = R(\vc{s}_0, \vc{a}) + \gamma \mathbb{E}_{\vc{s}_1{\sim}T(\vc{s}_0, \vc{a})}[V(\vc{s}_1)],
\end{equation}
which estimates the return of a trajectory starting with taking action $\vc{a}$ at state $\vc{s}_0$ and follows the policy $\pi_\theta$ afterwards. 

An optimal control policy $\pi_{\hat{\theta}}$ is defined as a policy that maximizes the expected Value Function value over the initial state distribution $\rho_0$:

\begin{equation}
\pi_{\hat{\theta}} = \arg\max_\pi \mathbb{E}_{\vc{s}{\sim}\rho_0}[V(\vc{s})].
\end{equation}

There is a large body of work in searching the optimal control policy using Reinforcement Learning\cite{}. In this work, we use Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, a state-of-the-art Policy Gradient algorithm, to learn the optimal control policy. PPO optimizes a modified objective to the original MDP problem:

\begin{align}
L_{PPO}({\theta}) = -\mathbb{E}_{\vc{s}_0, \vc{a}_0, \vc{s}_1, ...} [\min (&r(\theta)A_t, clip(r(\theta), 1-\epsilon, 1+\epsilon)A_t)],
\end{align}
where $r(\theta) = \frac{\pi_\theta(\vc{a}|\vc{s})}{\pi_{\theta_{old}}(\vc{a}|\vc{s})}$ is the importance re-sampling term that enables us to use data sampled under an old policy $\pi_{\theta_{old}}$ to estimate expectation for the current policy $\pi_{\theta}$, $\epsilon$ controls how much the probability ratio is clipped and $A_t=Q_t-V_t$ is the \textit{Advantage Function}. More details in deriving the objective functions can be found in the original paper of PPO. We chose PPO as the learning algorithm because it provides better data efficiency and learning performance than the alternative learning algorithms. Our method can also be easily applied to other learning algorithms such as Trust Region Policy Optimization (TRPO)\cite{} or Deep Deterministic Policy Gradient (DDPG)\cite{}.

Incorporating the Mirror Symmetry Loss, the final optimization problem for learning the locomotion policy can be defined as:

\begin{equation}
\pi_{\hat{\theta}} = \arg \min_\theta (L_{PPO}(\theta) + \omega_{mirror} L_{mirror}(\theta)),
\end{equation}
where $\omega_{mirror}$ is the weight of the Mirror Symmetry Loss. We use $\omega_{mirror} = 4$ for all the examples.

\section{Locomotion Curriculum}
\label{sec:loc_cur}

Although the Assistance Controller enables stable learning of locomotion controllers, the learned control policy usually does not work well without assistance. To obtain a control policy fully in 3D, we need a method to remove the dependency on the Assistance Controller. To design such a method, we need to answer two questions: when should the strength of the Assistance Controller be remove, and how much should it be remove, if not all at once. This turns out to be a non-trivial task, as an aggressive curriculum that reduces the assistance strength frequently usually leads to sub-optimal behaviors such as standing still or losing balance, while a conservative curriculum usually causes inefficiency in learning.

In this work, we design a learning curriculum that is empirically both stable and efficient. The learning curriculum consists of two components: the simulation-level curriculum and the learning-level curriculum. 

For each rollout during the simulation, we drop the Assistance Controller strength for a fixed percentage $k\%$ every $d$ seconds. This allows the policy to be robust to assistances with different strength, which prepares it for the subsequent drops in curriculum at the learning level. In addition, since the curriculum is discrete in time throughout the rollouts, they can be viewed as milestones for the policy to determine whether it has mastered certain curriculum strength.

At the learning level, we evaluate the performance of the policy and reduce the strength of the Assistance Controller when it successfully operates under the current setting. We use two metrics to define a successful policy. The first metric is that the policy needs to be able to balance the character for at least $2d$ seconds. As discussed above, this is to measure whether the policy is able to reach the second milestone during each rollout. The issue with using this metric alone is that the policy might learn to stand still, or move in a slow but balanced manner, which would easily satisfy the metric. To alleviate this problem, we also require the average return of the policy to reach a pre-determined threshold $T_{c}$, which should not be achievable for a standing-still policy. In all of our experiments, we set $d=3s$, $k=25$ and $T_c$ to be $70\%$ of the return from the initial policy trained with full assistance.

When the policy satisfies the two metrics defined above, we reduce the strength of the Assistance Controller also by $k\%$, similar to the simulation-level curriculum. Another way to see this update is that we now initialize the character from the second curriculum milestone instead of the first one.












==> overview.tex <==
\section{OVERVIEW}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/overview}
  \caption{Overview of our method. Black arrow denotes simulation steps, red arrow denotes information flow and blue arrow denotes learning steps.}
  \label{fig:overview}
\end{figure}

Figure \ref{fig:overview} shows an overview of our method, demonstrating how the locomotion curriculum and the mirror symmetry loss are incorporated into a standard reinforcement learning framework. 

At each simulation step, the simulator takes in a sampled action from the control policy and an assistance force produced by the Assistance Controller, and advances the character to the next timestep. It outputs the reward it receives and the new state $\vc{s}'$, which are then fed back to the two controllers to compute the control signal for the next step, as well as stored in a Data Buffer. 

When the data buffer has collected enough simulation samples, they will be used to compute updates to the control policy and the Assistance Controller. We use Policy Gradients method, and in particular Proximal Policy Optimization (PPO) to update the control policy, which maximizes the expected total reward of each trajectory. We augment the original PPO objective function with the Mirror Symmetry Loss, which guides the learning of a symmetric control strategy. Once the character learns to successfully move under the current setting, we update the Assistance Controller to provide less assistance. This loop continues until the character learns a fully 3D locomotion controller.















